Let's Talk This Out: Towards Explanation-based Distributed Goal Satisfaction

Digital systems are embedded in a modular environment of different components with individual goals and settings, which are often installed without central oversight. In this research preview paper we present a framework for communication between components to facilitate compositional problem solving based on explanation patterns and A/G-contracts, without the need for an oracle. Our approach uses partial MaxSMT solving and quantifier elimination to compute counterfactual explanation messages. We illustrate the feasibility of the approach with a proof-of-concept chain topology example, and discuss future challenges when expanding the protocol to more complex topologies.

==> eptcsdata.tex <==
\providecommand{\firstpage}{127}
\providecommand{\publicationstatus}{Matt Luckcuck, Maike Schwammberger, \& Akhila Bairy (Eds.):\\
Eighth International Workshop on Formal Methods\\
for Autonomous Systems (FMAS 2026)\\
EPTCS 457, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.457.9}{10.4204/EPTCS.457.9}}
\pdfoutput=1

